Lessons and Open Questions from a Unified Study of Camera-Trap Species Recognition Over Time

Camera traps are vital for large-scale biodiversity monitoring, yet accurate automated analysis remains challenging due to diverse deployment environments. While the computer vision community has mostly framed this challenge as cross-domain generalization, this perspective overlooks a primary challenge faced by ecological practitioners: maintaining reliable recognition at the fixed site over time, where the dynamic nature of ecosystems introduces profound temporal shifts in both background and animal distributions. To bridge this gap, we present the first unified study of camera-trap species recognition over time. We introduce a realistic benchmark comprising 546 camera traps with a streaming protocol that evaluates models over chronologically ordered intervals. Our end-user-centric study yields four key findings. (1) Biological foundation models (e.g., BioCLIP 2) underperform at numerous sites even in initial intervals, underscoring the necessity of site-specific adaptation. (2) Adaptation is challenging under realistic evaluation: when models are updated using past data and evaluated on future intervals (mirrors real deployment lifecycles), naive adaptation can even degrade below zero-shot performance. (3) We identify two drivers of this difficulty: severe class imbalance and pronounced temporal shift in both species distribution and backgrounds between consecutive intervals. (4) We find that effective integration of model-update and post-processing techniques can largely improve accuracy, though a gap from the upper bounds remains. Finally, we highlight critical open questions, such as predicting when zero-shot models will succeed at a new site and determining whether/when model updates are necessary. Our benchmark and analysis provide actionable deployment guidelines for ecological practitioners while establishing new directions for future research in vision and machine learning.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Camera traps have become a critical tool for ecology and conservation: they non-invasively capture large volumes of time-stamped images in natural habitats, supporting biodiversity monitoring, behavior analysis, and conservation planning~\cite{pollock2025harnessing,tuia2022perspectives}. Yet diversity in conditions across space and time---together with hardware and deployment variability---induces large shifts in image content, quality, and appearance~\cite{koh2021wilds,beery2021iwildcam}.  poses unique challenges for developing vision models, and addressing them is essential for accurate, automated analysis at ecological scales.

\begin{figure}[t]
\small
\centering
\noindent\includegraphics[width=\linewidth]{ECCV_2026/figures/1_teaser_sample_4.pdf}
\vskip -5pt
\caption{\small {Variability of camera-trap images across space and time. Each row shows the images of one camera. Top: season changes affect the environment and animal appearance; Middle: weather changes affect the habitats and where animals show up; Bottom: species distribution changes over time.}}
%\caption{\small {Variability of camera-trap images across space and time: top: season changes affect both environments/animals; middle: weather changes affect appearances of the same animal/scene; bottom: similar conditions can still yield different animals.}}
% , with pie charts representing the image distributions across species.
\vspace{-5mm}
\label{fig:overview}
\end{figure}

Prior studies have often framed the problem as standard domain adaptation and generalization~\cite{sagawa2021extending,koh2021wilds,zhou2022domain}, transferring models from source cameras or periods to unseen targets. While this positions camera traps as a testbed for machine learning robustness, it overlooks a deployment reality: {end users (\eg, ecological researchers, conservation practitioners) typically value \textbf{site-specific reliability over time} more than cross-domain leaderboards.} In practice, data arrive sequentially under changing field conditions. This casts camera-trap species recognition as an inherent \textbf{online continual learning (OCL)} problem~\cite{mai2022online}: models should be evaluated in chronological order and optionally updated as streams evolve, rather than assuming IID target data.


\iffalse
\begin{figure*}[t]
\centering
\noindent\includegraphics[width=0.575\linewidth]{example-image-a}
\caption{\textbf{Online continual learning scenario for camera traps}.} 
\label{fig:overview}
\end{figure*}
\fi

\emph{To study this practical setting, we contribute a benchmark, analyses, baseline evaluation, and open questions.}

\noindent\textbf{Benchmark design.} We target \textbf{camera-trap species classification over time}. For each camera, the image stream is decomposed into chronological \textbf{time intervals}. At step $j$, a model may be updated on interval $j$ and is then evaluated on $(j+1)$, following OCL protocol~\cite{mai2022online}. The benchmark builds on LILA BC~\cite{LILA-BC}, identifying $546$ cameras across $17$ datasets with at least $6$ months of data. We develop a unified, reproducible pipeline adhering to FAIR principles (Findable, Accessible, Interoperable, and Reusable) to standardize data, labels, and metadata, enabling others to convert additional camera-trap data into compatible streams.



% \begin{figure}[t]
% \small
% \centering
% \noindent\includegraphics[width=0.9\linewidth]{WACV_2026/figs/fig_1.png}
% \vskip -5pt
% \caption{\small {Illustration of the variability of camera trap images across space (different rows) and time (different columns)}, with pie charts representing the image distributions across species.} 
% \vskip -10pt
% \label{fig:overview}
% \end{figure}

\noindent\textbf{Data analysis.} On our streams, many cameras exhibit pronounced temporal shift (\eg, changes in species distribution), while each interval is often low-shot with severe class imbalance. Because camera traps acquire images passively, scaling data is slow---researchers must wait for animals to appear, and many species may not be observed within a given window~\cite{tu2023holistic}. These make naive adaptation brittle.

%We note that these issues can hardly be addressed by scaling up data, because camera trap acquire images passively. Researchers must wait for animals to appear, and not all species are observed within a given window~\cite{tu2023holistic}. These characteristics make naive adaptation brittle.

% Unlike web-scale settings, passively acquired images limit rapid data expansion: researchers must wait for animals to appear, and not all species are observed within a given window~\cite{tu2023holistic}. These characteristics make naïve adaptation brittle.

\noindent\textbf{Baseline analysis.} We study three reference strategies:
\begin{itemize}%[nosep,topsep=4pt,parsep=0pt,partopsep=4pt, leftmargin=*]
\item \textbf{Zero-shot} via BioCLIP-2~\cite{gu2025bioclip,stevens2024bioclip}, a recent vision foundation model trained on biological data.\footnote{BioCLIP 2~\cite{gu2025bioclip} achieves state-of-the-art zero-shot accuracy across various biodiversity datasets, including subsets of the LILA BC repository.} %\newnote{Zero-shot results for other models are provided in the Appendix.}
\item \textbf{Oracle} fine-tuning on all training data across intervals, assuming full a priori access to the stream (upper bound).
\item \textbf{Accumulated} fine-tuning using data from the current and all past intervals, representing a continually adaptative model without memory constraint.
\end{itemize}
We observe: (i) long-tailed zero-shot performance across the {$546$} cameras---over $170$ exceed 90\% accuracy, yet $169$ fall in $50–80\%$---indicating both promise and persistent cross-site difficulty; (ii) even with domain-specific data, naive oracle fine-tuning with a linear head does not consistently beat zero-shot, underscoring the challenge under limited data and severe imbalance; and (iii) a non-negligible gap between oracle and accumulated models---especially early in the stream---highlighting the difficulty of temporal shift and the need for online continual learning.

\noindent\textbf{Methods probe.} We evaluate several techniques for improving performance---parameter-efficient fine-tuning~\cite{mai2025lessons,xin2024parameter}, class-imbalance losses~\cite{ren2020balanced,ye2020identifying}, model-weight interpolation~\cite{ wortsman2022robust}, and post-hoc calibration~\cite{mai2024fine}. 
Results show both promise and limits under evolving streams, pointing to open machine learning questions for future work.
%{\color{red} Harry: In later sections, maybe study correlations between the proposed difficulty metrics and model performance, see if they can be used as practical tools for anticipating model reliability before deployment.}

\noindent\textbf{Practical analysis.} We further examine three questions from an end-user perspective: \emph{Will a zero-shot model suffice at a new site? If not, how much data are needed to adapt? Must we update continually to remain reliable?} Our study suggests: (1) deciding \emph{a priori} when zero-shot suffices is difficult without labeled feedback; (2) halting updates often degrades long-term performance; and (3) updating every interval is not uniformly beneficial---motivating data-driven when-to-adapt rules. These findings highlight practical research directions for robust model deployment in real-world ecological monitoring.

\noindent\textbf{Audiences.}
We provide a deployment-oriented benchmark and an empirical playbook for two communities:
\begin{itemize}%[nosep,topsep=4pt,parsep=0pt,partopsep=4pt, leftmargin=*]
\item \textbf{End users}: practical guidance on leveraging foundation models and lightweight updates for reliable, automated camera-trap analysis.
\item \textbf{Algorithm developers}: a realistic online continual learning (OCL) testbed to evaluate \emph{when to update} (triggers), \emph{what to retain} (small replay buffers), \emph{how to stay calibrated} over time, and \emph{how to learn under drift} (shift-aware objectives), under field constraints (scarce/imbalanced data, limited memory/compute, non-stationary streams).
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% OLD
\iffalse
Camera traps have become a critical tool in ecological and wildlife research for their ability to non-invasively capture large volumes of time-stamped images in natural habitats. These images provide rich, real-world data that support biodiversity monitoring, species behavior analysis, and conservation planning~\cite{pollock2025harnessing,tuia2022perspectives}. However, the diversity in environmental conditions across space and time, along with variations in hardware and deployment strategies, leads to significant variability in image content, quality, and appearance \cite{koh2021wilds,beery2021iwildcam}. This poses unique challenges for developing computer vision models, and addressing them is essential for enabling accurate, automated analysis at ecological scales.

Prior studies have often framed the problem through the lens of domain adaptation and generalization, aiming to transfer models trained on images from certain source domains (\eg, specific cameras or periods) to unseen target domains~\cite{sagawa2021extending,zhou2022domain}. While this perspective casts camera trap data as a novel testbed for existing machine learning challenges, it largely overlooks the practical needs of ecological researchers and conservation practitioners. These end users are typically less concerned with cross-domain performance benchmarks and more focused on maintaining reliable model performance in their specific deployment scenarios---as new data arrive over time in dynamic and evolving field conditions. These practical deployment considerations cast camera-trap species recognition as an inherent online continual learning problem---models are evaluated as new data arrives and are continually updated afterward, if needed. This approach sharply contrasts with prior studies that typically disregard the chronological structure of the data. 


To study this practical setting, we make the following contributions, including a benchmark, detailed analysis, and the proposal of several open questions. 

\noindent \textbf{Benchmark design.} We introduce a benchmark that targets \textbf{camera trap species classification over time}, designed to better reflect the real-world use of camera traps. We decompose the image stream from each camera into a sequence of \textbf{time intervals} based on timestamps and formulate the task as an instance of \textbf{online continual learning}~\cite{mai2022online}. At each time step $j$, a model is (optionally) updated using the training data from the $j$-th interval and then evaluated on the test data from the subsequent $(j+1)$-th interval.
To construct the benchmark, we build on the LILA BC repository~\cite{LILA-BC} and identify {$546$ camera traps from $17$ datasets, each with sufficient data spanning at least $6$ months.} We further develop a modular, reproducible data preparation pipeline that adheres to the FAIR principles (Findable, Accessible, Interoperable, and Reusable), enabling future researchers to convert their own camera trap data into similar benchmarks.

\noindent \textbf{Data analysis.} Building on our new benchmark, we first conduct a comprehensive analysis to better understand the underlying data characteristics. We find that image streams of many camera traps exhibit severe temporal shifts (\eg, species distributions) while each time interval contains severe class imbalance and limited images. We note that these questions cannot be addressed simply by scaling up data collection, as data collection in this domain is uniquely constrained---unlike many other applications, camera trap images are obtained passively, requiring researchers to wait for animals to appear in front of cameras, which can take days or even months. Moreover, not all relevant species may be observed during that time period, further complicating model adaptation~\cite{tu2023holistic}.


\noindent \textbf{Baseline analysis.} We evaluate three baseline methods:
\begin{itemize}[nosep,topsep=4pt,parsep=0pt,partopsep=4pt, leftmargin=*]
\item \textbf{Zero-shot}: classification using BioCLIP 2~\cite{gu2025bioclip,stevens2024bioclip}, a recent vision foundation model trained on biological data.\footnote{BioCLIP 2~\cite{gu2025bioclip} achieves state-of-the-art zero-shot performance across various biodiversity datasets, including subsets of the LILA BC repository.} \jy{In later sections, have a table for other models to show that BioCLIP 2 has the best overall zero-shot performance on your data, as in the BioCLIP 2 paper, we only used 5 camera trap datasets.}
\item \textbf{Oracle}: a reference model fine-tuned using all available training data from all time intervals, representing an upper-bound performance---the model is allowed to preview the entire image stream before training. 
\item \textbf{Accumulated}: a continually fine-tuned model trained on data from the current and all previous intervals, representing an adaptive method without memory constraints.
\end{itemize}

Our analyses yield several key findings. First, BioCLIP 2 zero-shot accuracy exhibits a long-tailed distribution across the {$546$} camera traps: over {$170$} achieve accuracy above {$90\%$}, demonstrating the promise of vision foundation models, while another {$169$} fall in the {$50\sim80\%$} range, highlighting the persistent need for adaptation. Second, despite access to domain-specific training data, naively fine-tuning BioCLIP 2 in the oracle setting (with a linear head) does not consistently outperform the zero-shot model. These underscore challenges in model fine-tuning and generalization in practical scenarios, especially under limited data and sever class imbalance. Third, there is a nonnegligieable gap between the oracle model and accumulated model, especially in early intervals, implying the challgende in temporal shift. 

We explore several machine learning techniques aimed at improving performance on our benchmark. {These include parameter-efficient fine-tuning~\cite{mai2025lessons,xin2024parameter}, loss functions for class imbalance~\cite{ren2020balanced,ye2020identifying}, model weight interpolation~\cite{wortsman2022robust}, post-processing logit calibration~\cite{mai2024fine}, and out-of-distribution detection~\cite{yang2024generalized}.} Our experiments reveal both the potential and limitations of these methods in the context of temporally evolving camera trap data.
{\color{red} Harry: In later sections, maybe study correlations between the proposed difficulty metrics and model performance, see if they can be used as practical tools for anticipating model reliability before deployment.}



\noindent \textbf{Practical analysis.}
Beyound these anaalysis and investigation, we take a end-user's perspeive to exlore several praxtical aspects. In practice, they face pressing questions before deployment: \emph{Will the model work well on data from a new location? If not, how much new data is needed to adapt it? And will the model require continual updates to remain effective?} Our findings are: 1)it is hard to determine when a zero-shot model is sufficient to be directly deployed without labeled test data, 2) halting adaptation often leads to performance degradation---suggesting the importance of continual updates in long-term deployments, 3) adapting models at every intervals not necessarily lead to imporvement, making it a question to deterimine when and how. 
These findings highlight promising future directions and open challenges for developing more robust, adaptive models in real-world ecological monitoring settings.


\noindent \textbf{Remark.} We present a novel benchmark for camera trap species classification over time, specifically designed to better reflect real-world deployment scenarios in ecological monitoring. Our work serves two primary audiences:
\begin{itemize}[nosep,topsep=4pt,parsep=0pt,partopsep=4pt, leftmargin=*]
\item \textbf{End-users} (e.g., ecological researchers and conservation practitioners): our benchmark and analyses provide practical guidance on how to leverage accessible models and tools for accurate, automated analysis of camera trap data.
\item \textbf{Algorithm developers} (e.g., computer vision and machine learning researchers): our benchmark offers a realistic testbed for developing and evaluating robust, adaptive models in an online continual learning setting, tailored to dynamic, real-world environments.
\end{itemize}
\fi



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Camera traps have become a critical tool in ecological and wildlife research for their ability to non-invasively capture large volumes of time-stamped images in natural habitats. These images provide rich, real-world data that support biodiversity monitoring, species behavior analysis, and conservation planning~\cite{pollock2025harnessing,tuia2022perspectives}. However, the diversity in environmental conditions across space and time, along with variations in hardware and deployment strategies, leads to significant variability in image content, quality, and appearance \cite{koh2021wilds,beery2021iwildcam}. This poses unique challenges for developing computer vision models, and addressing them is essential for enabling accurate, automated analysis at ecological scales.

%Prior studies have often framed the problem through the lens of domain adaptation and generalization, aiming to transfer models trained on images from certain source domains (\eg, specific cameras or periods) to unseen target domains~\cite{sagawa2021extending,zhou2022domain}. While this perspective casts camera trap data as a novel testbed for existing machine learning challenges, it largely overlooks the practical needs of ecological researchers and conservation practitioners. These end users are typically less concerned with cross-domain performance benchmarks and more focused on maintaining reliable model performance in their specific deployment scenarios as new data arrive over time in dynamic and evolving field conditions. In practice, they face pressing questions before deployment: \emph{Will the model work well on data from a new location? If not, how much new data is needed to adapt it? And will the model require continual updates to remain effective?} Importantly, data collection in this domain is uniquely constrained---unlike many other applications, camera trap images are obtained passively, requiring researchers to wait for animals to appear in front of cameras, which can take days or even months. \jy{Maybe first highlight that it is inherently an online continual learning problem, but there weren't any practice on this setting.} Moreover, not all relevant species may be observed during that time, further complicating model adaptation and evaluation~\cite{tu2023holistic}.

%To this end, we introduce a novel benchmark that targets \textbf{camera trap species classification over time}, designed to better reflect the real-world use of camera traps. We decompose the image stream from each camera into a sequence of \textbf{time intervals} based on timestamps and formulate the task as an instance of \textbf{online continual learning}~\cite{mai2022online}. At each time step $j$, a model is (optionally) updated using the training data from the $j$-th interval and then evaluated on the test data from the subsequent $(j+1)$-th interval. This setup mimics the practical deployment scenario, where models are evaluated as new data arrives and are incrementally updated afterward, if needed.
% This setup mimics the practical deployment scenario, where models are evaluated as new data becomes available and may be incrementally updated over time, if necessary. To construct the benchmark, we build on the LILA BC repository~\cite{LILA-BC} and identify {$546$ camera traps from $17$ datasets, each with sufficient data spanning at least $6$ months.} We further develop a modular, reproducible data preparation pipeline that adheres to the FAIR principles (Findable, Accessible, Interoperable, and Reusable), enabling future researchers to convert their own camera trap data into similar benchmarks.

\iffalse
Building on our new benchmark, we first conduct a comprehensive analysis to better understand the underlying data characteristics and the performance of baseline methods. To quantify the difficulty of each camera trap's image stream, we develop a set of metrics, including temporal shifts, class imbalance, and the emergence of novel species over time. 
%Importantly, data collection in this domain is uniquely constrained---unlike many other applications, camera trap images are obtained passively, requiring researchers to wait for animals to appear in front of cameras, which can take days or even months. \jy{Maybe first highlight that it is inherently an online continual learning problem, but there weren't any practice on this setting.} Moreover, not all relevant species may be observed during that time, further complicating model adaptation and evaluation~\cite{tu2023holistic}.

In practice, they face pressing questions before deployment: \emph{Will the model work well on data from a new location? If not, how much new data is needed to adapt it? And will the model require continual updates to remain effective?}


We then evaluate three baseline methods:
\begin{itemize}[nosep,topsep=4pt,parsep=0pt,partopsep=4pt, leftmargin=*]
\item \textbf{Zero-shot}: classification using BioCLIP 2~\cite{gu2025bioclip,stevens2024bioclip}, a recent vision foundation model trained on biological data.\footnote{BioCLIP 2~\cite{gu2025bioclip} achieves state-of-the-art zero-shot performance across various biodiversity datasets, including subsets of the LILA BC repository.} \jy{Maybe also have a table for other models, and show that BioCLIP 2 has the best overall zero-shot performances on your data, as in the BioCLIP 2 paper, we only used 5 camera trap datasets.}
\item \textbf{Oracle}: a reference model fine-tuned using all available training data from all time intervals, representing an upper-bound performance---the model is allowed to preview the entire image stream before training. 
\item \textbf{Accumulated}: a continually fine-tuned model trained on data from the current and all previous intervals, representing an adaptive method without memory constraints.
\end{itemize}

Our analyses yield three key findings. First, BioCLIP 2 zero-shot accuracy exhibits a long-tailed distribution across the {$546$} camera traps: over {$170$} achieve accuracy above {$90\%$}, demonstrating the promise of vision foundation models, while another {$169$} fall in the {$50\sim80\%$} range, highlighting the persistent need for adaptation. Second, despite access to domain-specific training data, the accumulated model does not consistently outperform the zero-shot model in early intervals. Sometimes, even the oracle model underperforms the zero-shot model. \jy{This may be true. But from figure 2, I don't see a very large gap. And the accumulated model is only obviously worse than zero-shot at interval 3.} These underscore challenges in model training and generalization in practical scenarios. %under limited data.  
Third, while the accumulated model eventually approaches the oracle model after sufficient intervals, halting adaptation leads to performance degradation---suggesting the importance of continual updates in long-term deployments. %{\color{red}Finally, we find non-negligible correlations between the proposed difficulty metrics and model performance, indicating their potential as practical tools for anticipating model reliability prior to deployment.}

In addition to baseline analyses, we explore several machine learning techniques aimed at improving performance on our benchmark. {These include parameter-efficient fine-tuning~\cite{mai2025lessons,xin2024parameter}, loss functions for class imbalance~\cite{ren2020balanced,ye2020identifying}, model weight interpolation~\cite{wortsman2022robust}, post-processing logit calibration~\cite{mai2024fine}, and out-of-distribution detection~\cite{yang2024generalized}.} Our experiments reveal both the potential and limitations of these methods in the context of temporally evolving camera trap data. These findings highlight promising future directions and open challenges for developing more robust, adaptive models in real-world ecological monitoring settings.

\noindent \textbf{Contributions.} We present a novel benchmark for camera trap species classification over time, specifically designed to better reflect real-world deployment scenarios in ecological monitoring. Our work serves two primary audiences:
\begin{itemize}[nosep,topsep=4pt,parsep=0pt,partopsep=4pt, leftmargin=*]
\item \textbf{End-users} (e.g., ecological researchers and conservation practitioners): our benchmark and analyses provide practical guidance on how to leverage accessible models and tools for accurate, automated analysis of camera trap data.
\item \textbf{Algorithm developers} (e.g., computer vision and machine learning researchers): our benchmark offers a realistic testbed for developing and evaluating robust, adaptive models tailored to dynamic, real-world environments.
\end{itemize}
\fi





==> tables_eccv/interval_length_sensitivity.tex <==
\begin{table}[tbh]
\vspace{3mm}
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setlength{\extrarowheight}{0pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{\hspace{2pt}}lcccccccccccc@{}}
\toprule
&
\cellcolor{col_color}C4 & C5
& \cellcolor{col_color}C7 & C8
& \cellcolor{col_color}C12 & C14
& \cellcolor{col_color}C15 & C16
& \cellcolor{col_color}C18 & C19
& \cellcolor{col_color}C20
& \multicolumn{1}{>{\columncolor{gray!15}}c}{Avg.} \\
\midrule

30-day ZS
& \cellcolor{col_color}\textbf{92.3} & 87.2
& \cellcolor{col_color}\textbf{82.6} & 82.1
& \cellcolor{col_color}80.2 & 79.3
& \cellcolor{col_color}77.9 & 76.5
& \cellcolor{col_color}75.3 & 69.5
& \cellcolor{col_color}62.7
& \multicolumn{1}{>{\columncolor{gray!15}}c}{78.9} \\

Accum$\star$
& \cellcolor{col_color}89.9 & \textbf{88.2}
& \cellcolor{col_color}81.0 & \textbf{83.0}
& \cellcolor{col_color}\textbf{85.4} & \textbf{90.7}
& \cellcolor{col_color}\textbf{84.9} & \textbf{80.9}
& \cellcolor{col_color}\textbf{80.0} & \textbf{79.6}
& \cellcolor{col_color}\textbf{75.4}
& \multicolumn{1}{>{\columncolor{gray!15}}c}{\textbf{83.6}} \\
\midrule
15-day ZS
& \cellcolor{col_color}\textbf{91.1} & 87.2
& \cellcolor{col_color}81.0 & 84.7
& \cellcolor{col_color}81.8 & 77.3
& \cellcolor{col_color}76.5 & 79.2
& \cellcolor{col_color}76.6 & 68.4
& \cellcolor{col_color}64.4
& \multicolumn{1}{>{\columncolor{gray!15}}c}{78.9} \\

15-day Accum$\star$
& \cellcolor{col_color}90.2 & \textbf{88.3}
& \cellcolor{col_color}\textbf{85.4} & \textbf{85.4}
& \cellcolor{col_color}\textbf{92.0} & \textbf{96.3}
& \cellcolor{col_color}\textbf{91.5} & \textbf{79.5}
& \cellcolor{col_color}\textbf{81.9} & \textbf{85.1}
& \cellcolor{col_color}\textbf{85.6}
& \multicolumn{1}{>{\columncolor{gray!15}}c}{\textbf{87.4}} \\
\midrule
60-day ZS
& \cellcolor{col_color}\textbf{92.4} & \textbf{82.8}
& \cellcolor{col_color}82.8 & \textbf{82.7}
& \cellcolor{col_color}80.1 & 81.3
& \cellcolor{col_color}82.7 & \textbf{76.2}
& \cellcolor{col_color}76.3 & 71.6
& \cellcolor{col_color}\textbf{69.4}
& \multicolumn{1}{>{\columncolor{gray!15}}c}{79.8} \\

60-day Accum$\star$
& \cellcolor{col_color}90.0 & 81.2
& \cellcolor{col_color}82.8 & 78.2
& \cellcolor{col_color}\textbf{87.0} & \textbf{83.4}
& \cellcolor{col_color}\textbf{84.6} & 72.3
& \cellcolor{col_color}\textbf{83.9} & \textbf{76.8}
& \cellcolor{col_color}66.2
& \multicolumn{1}{>{\columncolor{gray!15}}c}{\textbf{80.6}} \\
\bottomrule
\end{tabular}
}
\vspace{3mm}
\caption{\small Interval-length sensitivity on the evaluated camera subset. For both 15-day and 60-day intervals, accum$\star$ improves zero-shot in most cases.}
\label{tab:cl_interval}
\vspace{-5mm}
\end{table}

==> tables_eccv/wildclip.tex <==
\begin{table}[tbh]
\vspace{2mm}
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setlength{\extrarowheight}{0pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccccccccc}
\toprule
&
\cellcolor{col_color}C1 & C2
& \cellcolor{col_color}C3 & C4
& \cellcolor{col_color}C5 & C6
& \cellcolor{col_color}C8 & C9
& \cellcolor{col_color}C11 & C14
& \cellcolor{col_color}C16 & C17
& \cellcolor{col_color}C20
& \multicolumn{1}{>{\columncolor{gray!15}}c}{Avg.} \\
\midrule
ZS
& \cellcolor{col_color}80.7 & 68.6
& \cellcolor{col_color}90.5 & 52.6
& \cellcolor{col_color}\textbf{86.6} & 59.9
& \cellcolor{col_color}49.5 & \textbf{63.5}
& \cellcolor{col_color}76.0 & 57.8
& \cellcolor{col_color}46.2 & 76.3
& \cellcolor{col_color}64.2
& \multicolumn{1}{>{\columncolor{gray!15}}c}{67.1} \\

Accum
& \cellcolor{col_color}70.6 & 67.1
& \cellcolor{col_color}60.4 & 65.9
& \cellcolor{col_color}71.1 & 64.6
& \cellcolor{col_color}55.5 & 50.0
& \cellcolor{col_color}65.7 & 58.6
& \cellcolor{col_color}57.8 & 74.2
& \cellcolor{col_color}60.5
& \multicolumn{1}{>{\columncolor{gray!15}}c}{63.2} \\

Accum$\star$
& \cellcolor{col_color}\textbf{91.7} & \textbf{81.0}
& \cellcolor{col_color}\textbf{93.2} & \textbf{71.2}
& \cellcolor{col_color}79.2 & \textbf{73.9}
& \cellcolor{col_color}\textbf{67.8} & 59.2
& \cellcolor{col_color}\textbf{82.5} & \textbf{69.3}
& \cellcolor{col_color}\textbf{60.7} & \textbf{77.2}
& \cellcolor{col_color}\textbf{65.4}
& \multicolumn{1}{>{\columncolor{gray!15}}c}{\textbf{74.8}} \\
\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{\small \sy{Update the table number} WildCLIP results on the non-Serengeti camera subset. Serengeti cameras are excluded to avoid overlap with WildCLIP's training data.}
\label{tab:wildclip}
\end{table}
